A Computationally Efficient Sparsified Online Newton Method

Second-order methods hold significant promise for enhancing the convergence of deep neural network training; however, their large memory and computational demands have limited their practicality. Thus there is a need for scalable second-order methods that can efficiently train large models. In this paper, we introduce the Sparsified Online Newton (SONew) method, a memory-efficient second-order algorithm that yields a sparsified yet effective preconditioner. The algorithm emerges from a novel use of the LogDet matrix divergence measure; we combine it with sparsity constraints to minimize regret in the online convex optimization framework. Empirically, we test our method on large scale benchmarks of up to 1B parameters. We achieve up to 30% faster convergence, 3.4% relative improvement in validation performance, and 80% relative improvement in training loss, in comparison to memory efficient optimizers including first order methods. Powering the method is a surprising fact -- imposing structured sparsity patterns, like tridiagonal and banded structure, requires little to no overhead, making it as efficient and parallelizable as first-order methods. In wall-clock time, tridiagonal SONew is only about 3% slower per step than first-order methods but gives overall gains due to much faster convergence. In contrast, one of the state-of-the-art (SOTA) memory-intensive second-order methods, Shampoo, is unable to scale to large benchmarks. Additionally, while Shampoo necessitates significant engineering efforts to scale to large benchmarks, SONew offers a more straightforward implementation, increasing its practical appeal. SONew code is available at: https://github.com/devvrit/SONew

==> rebuttal.tex <==
% \begin{figure}[t!]
% \centering
% \begin{minipage}{0.8\textwidth}
%     \centering
%     \includegraphics[width=0.65\columnwidth]{figs/autoencoder_pytorch.png}
%     \label{fig:autoencoder_pytorch}
% \end{minipage}
% \caption{\small Autoencoder - Pytorch (NEW). We perform tridiag-SONew comparison with KFac [1], Eva [2], FishLeg [3] on the Autoencoder benchmark. We keep the batch size=1000 for all experiments. Eva is trained for 100 epochs, and for others we change number of epochs to train such that each experiment takes same amount of time. Each optimizer is tuned using 600 hyperparameters using NNI [4]. KFac and FishLeg optimizers' preconditioner is updated once every 10 steps. We observe that tridiagg-SONew beats all the baselines by large margin.}
% \label{fig:autoenc}
% \end{figure}

\begin{figure}[t!]
    % \begin{subfigure}
    \minipage{0.45\textwidth}
    \centering
    \caption*{\small (a) Autoencoder - Pytorch}
    \hfill\includegraphics[width=1.0\textwidth]{figs/autoencoder_pytorch.png}\hspace*{\fill}
    \label{fig:0b}
    \endminipage \hfill
    % \end{subfigure}\\
    % \begin{subfigure}
    \minipage{0.45\textwidth}
    \centering
    \caption*{\small (b) Autoencoder - JAX}
    \hfill\includegraphics[width=1.0\textwidth]{figs/autoencoder_time_plot.png}\hspace*{\fill}
    \label{fig:0b}
    \endminipage \hfill
    % \end{subfigure}
    \caption{\small (a) Autoencoder - Pytorch (NEW). We perform tridiag-SONew comparison with KFac [1], Eva [2], FishLeg [3] on the Autoencoder benchmark. We keep the batch size=1000 for all experiments. Eva is trained for 100 epochs, and for others we change number of epochs to train such that each experiment takes same amount of time. Each optimizer is tuned using 600 hyperparameters using NNI [4]. KFac and FishLeg optimizers' preconditioner is updated once every 10 steps. We observe that tridiagg-SONew beats all the baselines by large margin. (b) Comparison of optimizer which require $\leq 3*d$ parameters, where $d$ is the total number of parameters in the network. Note that we do not plot optimizers requiring much larger memory, like bds-4-SONew, Shampoo, rfdSON(4). This is because they're significantly slower (upto $5 \times$ slower) than first order methods on Autoencoder benchmark, since it's run on just one machine and there's no parallelism. Therefore, one needs to run them for only $\sim 20$ epochs to make them take similar time as first order methods. Since this is too less to make a fair comparison, we skip them here. We plot, though, Shampoo on OGBG where due to parallelized training, it's just upto $1.25\times$ slower (still considerably large, but much better than singe machine runs). As a result, one needs to run Shampoo for just $\sim 20\%$ fewer steps to run in similar time as other baselines and SONew.}
    \label{fig:large-benchmark-train}
\end{figure}



\begin{figure}[t!]
    % \begin{subfigure}
    \minipage{0.45\textwidth}
    \centering
    \caption*{\small (a) Valid. error rate on ViT}
    \hfill\includegraphics[width=1.0\textwidth]{figs/vit_error_rate_new.png}\hspace*{\fill}
    \label{fig:0b}
    \endminipage \hfill
    % \end{subfigure}\\
    % \begin{subfigure}
    \minipage{0.45\textwidth}
    \centering
    \caption*{\small (b) Valid. avg precoision on OGBG}
    \hfill\includegraphics[width=1.0\textwidth]{figs/ogbg_avg_prec_new.png}\hspace*{\fill}
    \label{fig:0b}
    \endminipage \hfill
    % \end{subfigure}
    \caption{\small Large Scale Benchmarks with Momentum and RmsProp baselines added. (a) VIT benchmark - Since all baselines take similar time, we plot performance wrt steps. (b) GraphNetwork benchmark - in the \Cref{fig:large-benchmarks}, we plotted performance wrt steps. Since Shampoo takes more time per step, we ran Shampoo on 80\% fewer steps, so that end-to-end time taken is same by all the optimizers. We observe that tridiag-SONew outperforms even Shampoo in wall clock time, while simultaneously taking much less memory.}
    \label{fig:large-benchmark-train}
\end{figure}

$[1]$ Martens et. al, 2015 Optimizing Neural Networks with Kronecker-factored Approximate Curvature \\
$[2]$ Eva: Practical Second-order Optimization with Kronecker-vectorized Approximation, ICLR 2023\\
$[3]$ Gracia et al., 2023 Fisher-Legendre (FishLeg) optimization of deep neural networks.\\
$[4]$ \href{https://nni.readthedocs.io/en/v2.3/Tuner/BuiltinTuner.html#Anneal}{https://nni.readthedocs.io/en/v2.3/Tuner/BuiltinTuner.html#Anneal}



% \begin{figure*}[!h]
%     \centering
%         \includegraphics[width=0.5\columnwidth]{images/de.drawio.pdf}
%         \caption{\small An illustration of the dual encoder modelling}
%         \label{fig:gc_dist_diagram}
%     \quad
% \end{figure*}
